MM-GEN: Enhancing Task Performance Through Targeted Multimodal Data Curation

Vision-language models (VLMs) are highly effective but often underperform on specialized tasks; for example, Llava-1.5 struggles with chart and diagram understanding due to scarce task-specific training data. Existing training data, sourced from general-purpose datasets, fails to capture the nuanced details needed for these tasks. We introduce MM-Gen, a scalable method that generates task-specific, high-quality synthetic text for candidate images by leveraging stronger models. MM-Gen employs a three-stage targeted process: partitioning data into subgroups, generating targeted text based on task descriptions, and filtering out redundant and outlier data. Fine-tuning VLMs with data generated by MM-Gen leads to significant performance gains, including 29% on spatial reasoning and 15% on diagram understanding for Llava-1.5 (7B). Compared to human-curated caption data, MM-Gen achieves up to 1.6x better improvements for the original models, proving its effectiveness in enhancing task-specific VLM performance and bridging the gap between general-purpose datasets and specialized requirements. Code available at https://github.com/sjoshi804/MM-Gen.

==> contents/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

\vb{make the arguments flow better:
1. Small VLMs are very appealing as they're cost effective and parameter efficient.
2. A key factor in developing such vlms that perform close to larger models is the data.
3. Today's VLMs are trained on large image-text pairs where textual descriptions are only high level and lack sufficient descriptive detail (add a figure showing an image with high-level desc and low-level detailed desc and ref to it here).
4. this in-turn results in models that have good performance in high-level img understanding tasks, but struggle in tasks that require more low-level details (can give brief ex of tasks here). 
5. Curating high-quality MM data which have low-level image details is an open problem.
6. A common approach to address this is to curate custom datasets by careful data selections and verifications for each task at hand. But this approach is expensive and time-consuming and non-trivial for a new setting.
7. In constrast in generative language models, automated data generation and annotation frameworks provide general recipes to synthetically generate data in new tasks.
8. Developing such automated frameworks for VLMs which can generate specialized, high quality data will enable large-scale and general data generation that can be applied broadly across tasks.
9. In this paper, we propose X -----
10. X contains, does, (some desc about your pipeline)
11. (the whole para on clip style embeddiings and long tail doesn't fit here, maybe needs to spread around in the previous passages.)
12. We show 1), 2), N)
13. We evaluate and show that X...
Our contributions are: ....}

\vv{To present a teaser image, we can start by showing a few examples, possibly taken from datasets like ChartQA or similar datasets. Next, we demonstrate various methods to generate captions, such as using traditional captioning models, web-sourced captions, and finally captions generated by our approach. Finally, we also show bar charts to highlight accuracy achieved using these different captioning methods.}

\sj{terminology:
curating v/s generating
text annotation as general term: caption / question as sepcific annotations?}

Small vision-language models (VLMs) are highly parameter-efficient, often over 100$\times$ smaller than their larger counterparts~\cite{llava,llava_ov}. Additionally, they achieve comparable performance on tasks requiring high-level image understanding, such as generating descriptive captions for images or recognizing central objects from an image~\cite{llava}. 
However, these models face challenges with tasks that require fine-grained understanding of details in the image\cite{vlmbenchmark, blink paper, eureka report}. Examples of such tasks include chart understanding, diagram interpretation, spatial reasoning. These challenges limit the deployment of more efficient smaller models in specialized contexts. \bn{Do we want to start the intro with a motivation on small models or do we think this is a more general method? Large vlms also face similar challenges, and targeted synthetic mm data generation has shown to be beneficial for larger models too. llama 405b was trained on a lot of synthetic data.}

The primary challenge is often the quality and the nature of the data. Data quality plays a crucial role in determining the performance of small models~\cite{phi1, phi5, phi3, orca1, orca2, orca3, llava}. Existing VLMs, especially smaller ones, are typically trained on large-scale datasets scraped from the internet, which contain broad, general-purpose image-text pairs or versions of \varun{versions of what? incomplete?}~\cite{?}. While this is sufficient for tasks that require on a high-level understanding of images e.g., describing what is happening in image generally \varun{``what is happening in image generally'' is not a very useful statement? maybe given another example? like the next one is nice? but it's unclear what a ``central'' object is}, identifying salient objects in an image, it falls short in specialized domains where a highly specific understanding of image details is essential \varun{example would be nice: one to contrast the "identifying central objects"}. A common approach to address these shortcomings is to curate custom datasets tailored to specific tasks, often with significant human effort: careful data source selection, highly human engineered prompts to use stronger VLMs' generations etc. for~\cite{mathllava, chartinstruct, peng2023kosmos2groundingmultimodallarge}.

%This includes \varun{prompt or caption?}, as seen in MathLLaVA~\cite{mathllava} and ChartInstruct~\cite{chartinstruct} amongst others. \sj{Expand a bit to include things like kosmos as well}. 
\varun{maybe rephrase this sentence to emphasize better that LLM land does not require human intervention? lead with that? the current sentence ``ends with it''. for example: In contrast, minimal human intervention is needed to minimize the gaps between small and large language models; this is supported by automated frameworks such as ..} On the other hand, for generative language models the analogous problem of small LMs lagging behind large LMs on specialized tasks has been tackled using automated frameworks such as AgentInstruct~\cite{orca3} that need little to no human supervision to generalize to new tasks. However, for VLMs, no such method exists and existing methods are not scalable in size \varun{what does size mean here?} or across tasks due to their dependence on human expertise.

In this paper, we propose a novel, scalable \varun{i would scrub scalable, since you used that word in the previous sentence?} method for \emph{curating multimodal data} to improve the performance of small vision-language models (VLMs) by leveraging supervision from stronger, more capable models. Specifically, we observe that obtaining relevant images is often not the primary bottleneck—methods such as Bing Image Search or CLIP-based retrieval from large open-source datasets can be highly effective for gathering a pool of relevant images. Instead, the main challenge lies in securing suitable text supervision for these images. Images often contain a diverse array of visual concepts, ranging from general (e.g. objects) to more specific (e.g., pairwise relations between objects, relative position of objects etc.). The details required for specialized tasks are often highly specific and typically reside in the long tail of these concepts \varun{you lost me with this ``long tail'' argument: why is it the case that it lies in the long tail? it's just that it's uncommon in the captioning?}. As a result, these details are less likely to appear in general-purpose captions sourced from the internet. \vv{Can we find a related paper that has studied distribution of captions on web-scale images or any other large datasets like LAION?} Even synthetic captioning approaches for general image descriptions, which are effective for training contrastive multimodal models like CLIP, do not solve this problem \varun{i would scrub the remainder of this sentence} when training VLMs on specialized tasks. While such approaches improve the syntactic structure and relevance of captions, they tend to overlook specific, infrequent details crucial for specialized tasks. For example, a general captioning model might label a food chain diagram simply as “a food chain of [x] ecosystem.” However, a VLM designed to support science education needs to recognize and describe critical details, such as the roles of each organism (e.g., producer, consumer, decomposer) and the directional flow of energy—information that is often missing from generic captions. 

To address this, we introduce \method, which generates detailed and highly-specific task-conditioned text \varun{caption?} for a given set of candidate images to provide more relevant multimodal supervision for VLMs on tasks requiring specialized image understanding. \bn{Need to get earlier to the contribution.}

First \varun{do you use a "second"?}, we empirically demonstrate that images in natural multimodal data \varun{what is ``natural'' multi-modal data?} act refer to several details and even in human curated text annotations many details may be omitted. As a result, general multimodal supervision fails to fully leverage the rich image information for task-specific performance. We also show that generating more descriptive general-purpose synthetic captions is insufficient for capturing task-specific details, due to the large volume of image information. \method{} tackles this problem by generating task-specific text conditioned on task descriptions, producing more relevant multimodal supervision. \varun{you use \method{} earlier; why introduce it now with the sentence ``then we present ..''?} Then, we present \method. \method{} takes as input: 1) a small set of reference multimodal samples for the task, 2) keywords representing the relevant types of images, and 3) a set of candidate images. It then employs a three-stage pipeline to generate high-quality synthetic text for the images: 1) partitioning data into subgroups, 2) generating targeted text based on the reference samples, and 3) filtering the data to reduce redundancy and discard outliers.

We evaluate \method{} across several challenging tasks \bn{mention which model}, including spatial reasoning, chart understanding, and diagram understanding. Our approach yields substantial absolute performance improvements of 29\%, 15\%, and 14\% on these tasks, respectively, following fine-tuning on \method-generated data. 
% To assess the effectiveness of our approach relative to human-curated i.i.d. training data, we fine-tuned models on such datasets to establish a \textit{skyline} benchmark. 
Comparing the gains achieved through \method{} to \textit{skyline} performance established by fine-tuning on human-curated i.i.d. training data, we find that \method{} reaches 0.4$\times$ and 0.5$\times$ of the skyline’s improvements in spatial reasoning and chart understanding, respectively. Notably, in diagram understanding, \method{} surpasses the skyline, achieving 1.6$\times$ the improvement. Additionally, we demonstrate that filtering up to 50\% of the generated data with a simple approach results in minimal performance loss and, in many cases, enhances overall performance. \bn{skyline has not been defined here}

\vb{General feedback on intro - overall good motivation and placing of your method. more details on proposed framework can help give some more clarity on how the method addresses the challenges - how does it reduce human effort, how is it general? Many details on limitations and challenges are repeated in different parts and can be cut down.}

\sj{some \# like x number of human hours to create this. etc. }

==> contents/1_v3_introduction.tex <==
\section{\sj{v3} Introduction}

Vision-language models (VLMs) have achieved remarkable performance on several coarse-grained understanding tasks \cite{llava}, they still struggle with tasks that require fine-grained understanding of details in images \cite{vlmbenchmark, blink paper, eureka report}. Examples of such tasks include chart understanding, diagram interpretation, spatial reasoning. These challenges limit the deployment of more efficient smaller models in specialized contexts.

The primary limitation for these smaller VLMs is the quality of the training data. In particular, the failure to provide supervision for learning visual details required for tasks relying on fine-grained image understanding. Existing VLMs are trained on large troves of image-caption data scraped from the internet. However, the vast majority of this data only provides coarse descriptions of the image. For example, consider the task of diagram understanding: for simplicity, focus only on questions about the relations between different entities in diagrams such as a food web. Web-scraped text annotation for `a diagram of a food web for fresh-water bodies' may simply be captioned with \texttt{`fresh-water food web'} as such text is often not very descriptive \cite{nguyen2024improving}. Such a `general' caption provides limited information overall and no supervision at all for fine-grained details in the image required for understanding the relations between different organisms in the food web. Thus, while small VLMs, trained on such data, may excel at coarse-grained descriptions of images, they fail on tasks relying on fine-grained visual information. 

Prior work in training contrastive multimodal models has also encountered the poor-quality of web-scraped image-caption data, and addressed them with more descriptive synthetically generated text annotations \cite{capsfusion,nguyen2024improving}. However, for tasks requiring fine-grained understanding, such annotations are often still insufficient. Images contain several visual details and it is extremely unlikely, even for highly descriptive annotations, to mention all these details. For example, a more descriptive synthetic caption for the food web may resemble: \texttt{an illustration showing the relationships between food web, food chain, and trophic levels in an aquatic ecosystem}. While more descriptive, such `general' synthetic captions are still likely to omit exact details necessary for the target task (e.g. the relationships between members of the food web are still not mentioned).

Thus, curating high-quality vision-language data that can provide supervision for the fine-grained details relevant for a particular task, remains challenging. While images for these tasks can be easily retrieved from large open-source image-caption datasets or using image search engines like Google or Bing, the challenge lies in obtaining text annotations referring to visual details relevant to the tasks. Recently, \cite{mathllava} curated such a specialized dataset aimed at multimodal mathematical question-answering. However, such approaches rely on significant human efforts; in particular, \cite{mathllava} involved careful curation of task-relevant image-question-answer data from existing multimodal math datasets and manual verification of synthetically generated annotations. Other recent work \cite{chartinstruct, zhang2024multimodalselfinstructsyntheticabstract} suffers from similar limitations. 

In contrast, for language models (LMs), highly general frameworks have been proposed to generate synthetic text for improving small models on specialized tasks, needing little to no human intervention \cite{phi1, phi15, phi3, orca1, orca2, orca3}. This enables easily scaling up the volume of data as well as generalizing to a variety of target tasks.

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{fig/placeholder.pdf}
\end{figure*}

To address this gap, we present \method, a highly general framework for synthesizing task-relevant text annotations for images. Our approach takes as input on 1) a small \# of reference samples from the target task 2) a list of types of images for this task 3) a candidate pool of images for which to generate text annotations. First, we partition the reference samples and candidate images using the provided list of image types. Then, for each subgroup in the partition, we provide a reference sample and a candidate image to a stronger VLM to generate text annotation for the candidate image for the task that is specified by the reference sample. Finally, we filter the resulting image-text pairs to prioritize examples with middle perplexity, eliminating examples that are already learned (low perplexity) or too hard (high perplexity) to learn for the small VLM. 

We evaluate the effectiveness of this framework on chart understanding and reasoning, diagram understanding and spatial reasoning on maps. The data curated by \method allows us to see an absolute improvement over the base Llava-1.5 of 15\%, 14\% and 29\%, respectively. We also see improvements over the base Phi3-V of \sj{add results \%}, respectively. Moreover, the simple filtering strategy we propose is extremely promising for VLMs, allowing for discarding up to 50\% data with no / minimal loss in performance. We also compare our method to 1) generating general text annotations - to highlight the importance of task-relevant text 2) task specified using natural language - to showcase how critical the data-centric approach to specifying the task is. Finally, we present ablations over key design choices in \method e.g. size of the reference sample set, generating with / without partitioning, scaling number of in-context samples. 

To summarize, we: 
\begin{enumerate}
    \item Present a highly general framework for multimodal data generation: \method
    \item Demonstrate  the importance of task-specificity in text annotations for images for tasks requiring fine-grained understanding \looseness=-1
    \item Establish the importance of data-centric descriptions of tasks for generating task-specific text annotations
    \item Propose a novel data-filtering scheme for VLMs that can reduce volume of training data by up to 50\%
\end{enumerate}

==> contents/theory.tex <==
\section{Theory / Formalism}

True Generative Process (mathematically, these will be vectors):
\begin{enumerate}
    \item Ground Truth: Modality Agnostic
    \item Image Data: \textbf{Dense} Noisy mapping from ground truth to image space \sj{nearly all features present in every image, to some extent}
    \item Text Data:  \textbf{Highly Sparse} mapping from ground truth to text space
\end{enumerate}

Generating high quality data that is dense can be quite difficult in general. Additionally, vision models are weaker (perhaps as a consequence of the previous statement). As a result, we select images that are somewhat similar i.e. we ensure that they sufficiently represent the ground truth concepts we care about and then we generate synthetic captions or QnA that target the concepts we care about in text space, thus, teaching the model the desired skill.  

Relevant related work: \cite{xue2024understandingrobustnessmultimodalcontrastive}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> todos.tex <==
\section{Plan}

\subsection{Finalizing Motivation / Pitch of Paper}

Two key elements of story: 
\begin{enumerate}
    \item Task-Specific Accompanying Text: 
    \begin{enumerate}
        \item Image modality has a lot of information, accompanying text is usually not as information dense
        \item Simply making captions more descriptive is insufficient, it may help provide supervision for more details in images but is still likely to miss \textbf{we show via baseline}
        \item \sj{add discussion on under-exploration of multimodal data, add more discussion on how images are not fully used yet}
        \item \sj{motivate partition from the very beginning}
        \item \sj{consider some baseline of what would happen if you keep scaling data up}
        \item \sj{argument of long-tail}
    \end{enumerate}
    \item Data-Centric Task Specification: Having established that it is necessary to limit the scope of accompanying text, how do we do this when using a stronger teacher model to generate accompanying text
    \begin{enumerate}
        \item Borrow motivation in part from \url{https://arxiv.org/abs/2211.09859}
        \item We can specify this targeting to stronger models via instructions or samples from the target task
        \item We show that following a data-centric approach to specifying the task description is far superior to using instructions: 
        \begin{enumerate}
            \item natural language instructions struggle to provide the precise targeting that even a few samples from the target task distribution can give. \textbf{would a baseline where we use the task description as the instruction be sufficient?}
            \item with access to a validation set for the desired task, this can be easily automated
        \end{enumerate}
    \end{enumerate}
\end{enumerate}

\subsection{Experiments}

Consolidating current results
\begin{enumerate}
    \item mminsturct + skyline \sj{add for Spatial Map on Llava}
    \item Generic Caption Baseline for All Datasets \sj{Add for SpatialMap, AI2D}
    \item Task Description / Task Specific Instruction Baseline  \sj{All Datasets}
    \item filtered runs \sj{add for Spatial Map, AI2D} \sj{first comute ppl and then select based on this}
    \item Ablations (to be done on ChartQA)
    \begin{enumerate}
        \item With and without partition using image type identifiers
        \item Ref Samples Set Quality
        \item \# of In-Context Samples Provided for Generation
        \item Scaling \# of Images v/s \# of Captions per Images for fixed budget of \# of Samples. 
    \end{enumerate}
    \item MMC - Evaluate on this dataset
\end{enumerate}

Getting further results
\begin{enumerate}
\item Next Tasks: OCRBench, MathVista (retry)
\item Next Models: Add result with 1 recent SOTA Vlm like Pixtral \sj{look at llama 3.2 vision 11B}, MOLMO
\end{enumerate}

\sj{I think we should frame this as a re-captioning work for generative VLMs in order to show the distinction of making things task specific over prior work.}

\sj{need to mention that there are many tasks that live in the long tail of multimodal data due to the density of information in images and sparsity of information in accompanying text}

\sj{New Intro Sketch:
\begin{enumerate}
    \item small vlm are v. efficient and great at general purpose image understanding but performance on task-specialized image understanding is still often lagging far behind larger models. \textbf{cite some numbers to prove this point}
    \item The challenge lies primarily in the distribution of the data that these models were trained on. In particular, Existing work has curated custom datasets to improve performance on such tasks, but with significant human involvement e.g. curating data sources, custom prompts etc. \textbf{cite mathllava, chartinstruct}
    \item In this paper, we leverage the supervision from a stronger model to generate data to solve this problem. While finding images relevant for this task can be relatively straightforward (e.g. Bing Image Search, CLIP-retrieval from large open-source datasets), the main bottleneck remains obtaining task-relevant text annotations that provide high quality supervision for the details in the image relevant to the task we care about. \url{https://github.com/UCSC-VLAA/Recap-DataComp-1B}
\end{enumerate}
}
